Underspecification Presents Challenges for Credibility in Modern Machine Learning

ML models often exhibit unexpectedly poor behavior when they are deployed in real-world domains. We identify underspecification as a key reason for these failures. An ML pipeline is underspecified when it can return many predictors with equivalently strong held-out performance in the training domain. Underspecification is common in modern ML pipelines, such as those based on deep learning. Predictors returned by underspecified pipelines are often treated as equivalent based on their training domain performance, but we show here that such predictors can behave very differently in deployment domains. This ambiguity can lead to instability and poor model behavior in practice, and is a distinct failure mode from previously identified issues arising from structural mismatch between training and deployment domains. We show that this problem appears in a wide variety of practical ML pipelines, using examples from computer vision, medical imaging, natural language processing, clinical risk prediction based on electronic health records, and medical genomics. Our results show the need to explicitly account for underspecification in modeling pipelines that are intended for real-world deployment in any domain.

==> sections/ehr_old.tex <==


\section{Case Study in Clinical Predictions from Electronic Health Records}
The rise of Electronic Health Record (EHR) systems has created an opportunity for building predictive ML models for diagnosis and prognosis (e.g. \cite{Ambrosino1995, Brisimi2019, Feng2019}).

In this section, we focus on one such model that uses a Recurrent Neural Network (RNN) architecture with EHR data to predict acute kidney injury (AKI) during hospital admissions \citep{Tomasev2019}. AKI is a common complication in hospitalized patients and is associated with increased morbidity, mortality, and healthcare costs \citep{Khwaja2012}.
Early intervention can improve outcomes in AKI~\citep{nice2019}, which has driven efforts to predict it in advance using machine learning. \cite{Tomasev2019} achieve state-of-the-art performance, detecting the onset of AKI up to 48 hours in advance with an accuracy of 55.8\% across all episodes and 90.2\% for episodes associated with dialysis administration. 

Despite this strong discriminative performance, there have been questions raised about what associations are being learned by this model and whether these conform with our understanding of physiology \citep{kellum2019artificial}.
Specifically, for some applications, it is desirable to disentangle physiological signals from operational factors related to the delivery of healthcare, both of which appear in EHR data.
As an example, the value of a lab test may be considered as a physiological signal; however the timing of that same test may be considered an operational one (e.g. due to staffing constraints during the night or timing of ward rounds).
Given the fact that operational signals may be institution-specific and are likely to change over time, understanding to what extent a model relies on different signals can help practitioners determine whether the model meets their specific generalization requirements \citep{futoma2020myth}. 

Here, we show that underspecification makes the answer to this question ambiguous. 
Specifically, we apply our experimental protocol to the \citet{Tomasev2019} AKI model which predicts the continuous risk (every 6 hours) of AKI in a 48h lookahead time window (see Appendix~\ref{sec:ehr appendix} for details).


\subsection{Data, model ensemble, and metrics}

The model and data used in this study are described in detail in \cite{Tomasev2019}. Briefly, the data consists of de-identified EHRs from 703,782 patients across multiple sites in the United States collected at the US Department of Veterans Affairs between 2011 and 2015. Records include structured data elements such as medications, labs, vital signs, diagnosis codes etc, aggregated in six hour time buckets (time of day 1: 12am-6am, 2: 6am-12pm, 3: 12pm-6pm, 4: 6pm-12am).
In addition, precautions beyond standard de-identification have been taken to safeguard patient privacy: free text notes and rare diagnoses have been excluded; many feature names have been obfuscated; feature values have been jittered; and all patient records are time-shifted, respecting relative temporal relationships for individual patients. Therefore, this dataset is only intended for methodological exploration.

The model consists of embedding layers followed by a 3 layer-stacked RNN before a final dense layer for prediction of AKI across multiple time horizons.
Our analyses focus on predictions with a 48h lookahead horizon, which have been showcased in the original work for their clinical actionability. 
To examine underspecification, we construct a model ensemble by training the model from 5 random seeds for each of three RNN cell types: Simple Recursive Units (SRU, \cite{Lei2018}), Long Short-Term Memory (LSTM, \cite{Hochreiter1997}) or Update Gate RNN (UGRNN, \cite{Collins2017}).
This yields an ensemble of 15 model instances in total.

The primary metric that we use to evaluate model performance is normalized area under the precision-recall curve (PRAUC) \citep{Boyd2012}, evaluated across all patient-timepoints where the model makes a prediction.
This is a PRAUC metric that is normalized for prevalence of the positive label (in this case, AKI events).
Our ensemble of models achieves tightly constrained normalized PRAUC values between 34.59 and 36.61.

\subsection{Reliance on operational signals}

In this dataset, the prevalence of AKI is largely the same across different times of day (see Table 1 of Supplement).
However, AKI is diagnosed based on lab tests, specifically a comparison of past and current values of creatinine \citep{Khwaja2012}, and there are clear temporal patterns in how tests are ordered.
For most patients, creatinine is measured in the morning as part of a `routine', comprehensive panel of lab tests.
Meanwhile, patients requiring closer monitoring may have creatinine samples taken at additional times, often ordered as part of an `acute', limited panel (usually, the basic metabolic panel\footnote{This panel samples Creatinine, Sodium, Potassium, Urea Nitrogen, CO2, Chloride and Glucose.}).
Thus, both the time of day that a test is ordered, and the panel of tests that accompany a given measurement may be considered as operational factors correlated with AKI risk. Note that neither of these factors are purely operational - there is known variation in kidney function across the day and the values of accompanying lab tests carry valuable information about patient physiology. However, we use these here as approximations for an operational perturbation.

To probe whether the model relies on these operational signals, we construct stress tests by applying two interventions to the test data that modify (1) the time of day feature and (2) the selection of lab tests.
The first intervention shifts the patient timeseries by a fixed offset, while the second intervention additionally removes all blood tests from time steps where creatinine is recorded, except for the basic metabolic panel.
We hypothesize that if the model encodes physiological signals rather than these operational cues, the predictions would be invariant to these interventions.
More importantly, if the model's reliance on these operational signals is underspecified, we would expect the behavior of the model instances in our ensemble to respond differently these modified inputs.

We begin by examining overall performance on this shifted test set across our ensemble.
In Figure~\ref{fig:ehr_shift_pop}, we show that performance on the intervened data is both worse and more widely dispersed than in the standard test set, especially when both interventions are applied.
This shows that the model incorporates time of day and lab content signals, and that the extent to which it relies on these signals is sensitive to both the recurrent unit and random initialization.

\begin{figure}[!ht]
    \centering
    \includegraphics{figures/EHR/EHR_population_shift_PRAUC.png}
    \caption{\textbf{Variability in performance from ensemble of RNN models processing electronic health records (EHR)}. Model sensitivity to time of day and lab perturbations.
    The x-axis denotes the evaluation set: ``Test'' is the original test set; ``Shift'' is the test set with time shifts applied; ``Shift + Labs'' applies the time shift and subsets lab orders to only include the basic metabolic panel CHEM-7.
    The y-axis represents the normalized PRAUC, and each set of dots joined by a line represents a model instance.}
    \label{fig:ehr_shift_pop}
\end{figure}

The variation between models is clearer when examining how these interventions affect risk predictions at individual patient-timepoints.
Here, we focus on the LSTM models whose aggregate performance was most and least affected by the time shift and lab intervention such that the only difference between these models is their random seeds.
We also focus on patient-timepoints at which creatinine measurements were taken.
In Figure~\ref{fig:ehr_shift_hist}~\textbf{b}, we show distributions of predicted risk on the original patient-timepoints observed in the ``early morning'' (12am-6am) time range, and proportional changes to these risks when the timeshift and lab interventions were applied.
Both models exhibit substantial changes in predicted risk under both interventions, with a wider range of changes when both interventions are applied.
However, the second model is far more sensitive to these changes than the first, with the predicted risks taking on substantially different distributions depending on the time range to which the observation is shifted.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/EHR/ehr_summary_shifts_tod1.png}
    \caption{\textbf{Variability in AKI risk predictions between two LSTM models processing electronic health records (EHR)}. Histograms showing showing risk predictions from two models, and changes induced by time of day and lab perturbations.
    Histograms show counts of patient-timepoints where creatinine measurements were taken in the early morning (12am-6am). LSTM 1 and 5 differ only in random seed.
    ``Test'' shows histogram of risk predicted in original test data.
    ``Shift'' and ``Shift + Labs'' show histograms of proportional changes (in \%) $\frac{\text{Perturbed} - \text{Baseline}}{\text{Baseline}}$ induced by the time-shift perturbation and the combined time-shift and lab perturbation, respectively.}
    \label{fig:ehr_shift_hist}
\end{figure}

These shifts in risk are consequential for decision-making and can result in AKI episodes being predicted tardily or missed.
In Figure~\ref{fig:ehr_shift_flipped}, we illustrate the number of patient-timepoints where the changed risk score crosses each model's calibrated decision threshold.
In addition to substantial differences in the number of flipped decisions, we also show that most of these flipped decisions occur at different patient-timepoints across models.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/EHR/Flipped_decisions.png}
    \caption{\textbf{Variability in AKI predictions between two LSTM models processing electronic health records (EHR)}.
    Counts (color-coded) of decisions being flipped due to the stress tests, from the LSTM 1 and LSTM 5 models, as well as the proportions of those flipped decision intersecting between the two models (in \%). Rows represent the time of day in the original test set, while columns represent the time of day these samples were shifted to. LSTM 1 and 5 differ only in random seed. ``Shift'' represents the flipped decisions (both positive to negative and negative to positive) between the predictions on the test set and the predictions after time-shift perturbation. ``Shift + Labs'' represents the same information for the combined time-shift and labs perturbation.}
    
    \label{fig:ehr_shift_flipped}
\end{figure}

\subsection{Conclusions}
We draw two major conclusions from these results.
First, given the model's current specification and training procedure, it tends to rely on the pattern of lab orders in the EHR data in a substantial way.
This may or may not present challenges in deployment, depending on how stable this signal is in the deployment context.
Secondly, and more importantly, the reliance on this signal is not \emph{enforced} by the model specification or training data.
As we have shown with our experimental protocol, even innocuous changes to the training procedure (here random seed and recurrent cell) are enough to push the trained model to incorporate this signal more or less in its predictions.
This suggests that, without major changes to the problem setup, invariances to certain signals could be enforced \emph{without sacrificing iid performance} by simply adding constraints to the training procedure, for example, by enforcing conditional independences implied by medical knowledge.
This is compatible with previous findings that inputting medical/domain relational knowledge has led to better out of domain behaviour \cite{Nestor2019}, performance \cite{Popescu2011, Choi2017, Tomasev2019, Tomasev2019a} and interpretability \cite{Panigutti2020} of ML models.
